O1 Replication Journey: A Strategic Progress Report -- Part 1

This paper introduces a pioneering approach to artificial intelligence research, embodied in our O1 Replication Journey. In response to the announcement of OpenAI's groundbreaking O1 model, we embark on a transparent, real-time exploration to replicate its capabilities while reimagining the process of conducting and communicating AI research. Our methodology addresses critical challenges in modern AI research, including the insularity of prolonged team-based projects, delayed information sharing, and the lack of recognition for diverse contributions. By providing comprehensive, real-time documentation of our replication efforts, including both successes and failures, we aim to foster open science, accelerate collective advancement, and lay the groundwork for AI-driven scientific discovery. Our research progress report diverges significantly from traditional research papers, offering continuous updates, full process transparency, and active community engagement throughout the research journey. Technologically, we proposed the journey learning paradigm, which encourages models to learn not just shortcuts, but the complete exploration process, including trial and error, reflection, and backtracking. With only 327 training samples and without any additional tricks, journey learning outperformed conventional supervised learning by over 8\% on the MATH dataset, demonstrating its extremely powerful potential. We believe this to be the most crucial component of O1 technology that we have successfully decoded. We share valuable resources including technical hypotheses and insights, cognitive exploration maps, custom-developed tools, etc at https://github.com/GAIR-NLP/O1-Journey.

==> learning-method-comparison.tex <==


\begin{table*}[!t]
    \centering
    \setlength{\tabcolsep}{6pt}
    {
    \fontsize{10}{13}\selectfont % 设置字体大小为10pt，行距为13pt
    \renewcommand\arraystretch{1.2}
    \resizebox{\linewidth}{!}{
        \begin{tabular}[l]{lll}
        \toprule
        \textbf{Characteristic} & \textbf{Shortcut Learning} & \textbf{Journey Learning} \\ \midrule
        \multirow{1}{*}{\textbf{Learning Objective}} & Quickly achieve specific tasks or metrics & Comprehensive deep understanding, continuous improvement \\ 
        \multirow{1}{*}{\textbf{Learning Depth}} & Surface features and simple correlations & Deep causal relationships and underlying principles \\ 
        \multirow{1}{*}{\textbf{Adaptability}} & Limited to specific tasks or data distributions & Broadly adaptable to different contexts and tasks \\ 
        \multirow{1}{*}{\textbf{Reasoning Ability}} & Limited, struggles with complex reasoning & Powerful, demonstrates human-like reasoning \\ 
        \multirow{1}{*}{\textbf{Self-Improvement}} & Lacks self-correction mechanisms & Continuous self-assessment and improvement \\ 
        \multirow{1}{*}{\textbf{Learning Process}} & Static, one-time training & Dynamic, continuous learning and adaptation \\ 
        \multirow{1}{*}{\textbf{Generalization}} & Limited, easily affected by data distribution changes & Strong, can handle new situations \\ 
        \multirow{1}{*}{\textbf{Innovation Capacity}} & Limited, struggles to solve new problems & High, can generate innovative solutions \\ 
        \multirow{1}{*}{\textbf{Data Dependency}} & Highly dependent on large training datasets & More focused on quality and learning strategies \\ 
        \multirow{1}{*}{\textbf{Computational Efficiency}} & Often requires significant computational resources & Potentially more efficient, focusing on strategy over scale \\ 
        \multirow{1}{*}{\textbf{Interpretability}} & Poor, often seen as a "black box" & Better, can track internal reasoning processes \\ 
        \multirow{1}{*}{\textbf{Ethical Considerations}} & May unintentionally amplify data biases & Easier to implement ethical constraints and adjustments \\ 
        \multirow{1}{*}{\textbf{Security}} & Vulnerable to adversarial attacks & More robust, able to identify potential threats \\ 
        \multirow{1}{*}{\textbf{Long-term Value}} & Quick results in specific tasks & Paves the way for AGI development \\ 
        \multirow{1}{*}{\textbf{Human Analogy}} & Exam-oriented education, crash courses & Comprehensive education, lifelong learning \\ 
        \bottomrule
        \end{tabular}
    }
    \caption{Comparison between Shortcut Learning and Journey Learning.}
    \label{tab:comparison}
    }
\end{table*}


